CUPre: Cross-domain Unsupervised Pre-training for Few-Shot Cell Segmentation

While pre-training on object detection tasks, such as Common Objects in Contexts (COCO) [1], could significantly boost the performance of cell segmentation, it still consumes on massive fine-annotated cell images [2] with bounding boxes, masks, and cell types for every cell in every image, to fine-tune the pre-trained model. To lower the cost of annotation, this work considers the problem of pre-training DNN models for few-shot cell segmentation, where massive unlabeled cell images are available but only a small proportion is annotated. Hereby, we propose Cross-domain Unsupervised Pre-training, namely CUPre, transferring the capability of object detection and instance segmentation for common visual objects (learned from COCO) to the visual domain of cells using unlabeled images. Given a standard COCO pre-trained network with backbone, neck, and head modules, CUPre adopts an alternate multi-task pre-training (AMT2) procedure with two sub-tasks -- in every iteration of pre-training, AMT2 first trains the backbone with cell images from multiple cell datasets via unsupervised momentum contrastive learning (MoCo) [3], and then trains the whole model with vanilla COCO datasets via instance segmentation. After pre-training, CUPre fine-tunes the whole model on the cell segmentation task using a few annotated images. We carry out extensive experiments to evaluate CUPre using LIVECell [2] and BBBC038 [4] datasets in few-shot instance segmentation settings. The experiment shows that CUPre can outperform existing pre-training methods, achieving the highest average precision (AP) for few-shot cell segmentation and detection.

==> tables/info-of-data-number.tex <==
\begin{table*}[]
\centering
\caption{An Overview of the Number of Images/Cells.}
\label{tab:number-info-of-image/cell}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
 & \multicolumn{10}{c}{\textbf{LIVECell} \cite{edlund2021livecell}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{BBBC038 \cite{caicedo2019nucleus}}}} \\
 \cmidrule(r){2-11}
 & \multicolumn{2}{c}{\textbf{Dataset-wide}} & \multicolumn{2}{c}{\textbf{SH-SY-5Y}} & \multicolumn{2}{c}{\textbf{MCF7}} & \multicolumn{2}{c}{\textbf{A172}} & \multicolumn{2}{c}{\textbf{BT474}} & \multicolumn{2}{c}{} \\
 \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}
 & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Cell} \\
 \midrule
Train-5\% & 162 & 51,256 & 22 & 6,837 & 24 & 10,969 & 20 & 4,526 & 22 & 4,032 & 34 & 1,753 \\
Train-10\% & 325 & 93,571 & 44 & 14,103 & 46 & 18,436 & 39 & 9,024 & 42 & 8,444 & 67 & 2,644 \\
Train-15\% & 487 & 149,410 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 100 & 3,770 \\
Train-20\% & 650 & 205,431 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 134 & 5,523 \\
\midrule
Train-100\% & 3,253 & 1,018,576 & 449 & 165,397 & 469 & 212,688 & 388 & 83,175 & 429 & 82,900 & 536 & 24,237 \\
\midrule
Valid & 570 & 181,610 & 79 & 28,199 & 82 & 39,252 & 68 & 15,688 & 75 & 14,526 & 67 & 2,905 \\
Test & 1,564 & 462,261 & 176 & 75,988 & 184 & 96,914 & 152 & 32,978 & 168 & 32,585 & 67 & 2,319 \\
\bottomrule
\end{tabular}
\end{table*}
